HDMapGen: A Hierarchical Graph Generative Model of High Definition Maps

High Definition (HD) maps are maps with precise definitions of road lanes with rich semantics of the traffic rules. They are critical for several key stages in an autonomous driving system, including motion forecasting and planning. However, there are only a small amount of real-world road topologies and geometries, which significantly limits our ability to test out the self-driving stack to generalize onto new unseen scenarios. To address this issue, we introduce a new challenging task to generate HD maps. In this work, we explore several autoregressive models using different data representations, including sequence, plain graph, and hierarchical graph. We propose HDMapGen, a hierarchical graph generation model capable of producing high-quality and diverse HD maps through a coarse-to-fine approach. Experiments on the Argoverse dataset and an in-house dataset show that HDMapGen significantly outperforms baseline methods. Additionally, we demonstrate that HDMapGen achieves high scalability and efficiency.

==> experiment_backup.tex <==
\section{Experiments}
In this section, we demonstrate the efficacy of our proposed \HDMapGen model to generate high quality maps. We explore three autoregressive generative models for sequence, plain graph and hierarchical graph input representations, and evaluate for generation quality, diversity and efficiency.

\subsection{Dataset and Implementation Details}

\PAR{Datasets.} We evaluate the performance of our models on two datasets across three cities in the US. One is the public Argoverse dataset \cite{chang2019argoverse}, which covers Miami (a total size of 204 kilometers of lanes) and Pittsburg (a total size of 86 kilometers). We sample 12000 maps with a field-of-view (FoV) of $200m \times 200m$ as the training dataset for Miami, and 5000 maps with the same FoV for Pittsburg. We also evaluate on an in-house dataset, which covers maps from the city of San Francisco. We train on $6000$ maps with a FoV of $120m\times120m$.

\PAR{Map Preprocessing}. %from Vectorized Data to Hierarchical Graph}
The key components of HD maps, the central line of drivable lanes, are usually over-sampled to guarantee a sufficient resolution. However, due to limitations in the scalability in graph neural networks, in a pre-processing step, we remove redundant control points with limited variation of curvature in each lane. This step enables us to remove an average of $70\%$ of points while not compromising the map quality. We define a hierarchical spatial graph based on the processed vector map. We use Depth-First-Search (DFS) to construct the adjacency matrix of global graph and define the generation order for the autoregressive model. 

\PAR{Implementation Details}.\HDMapGen uses graph attention neural network as the core part to perform the attentive message passing for graph inputs. We use multi-layer-perceptrons (MLPs) for all other encoding and decoding steps. The graph node coordinates are normalized to $[-1,1]$. The model is trained on a single Tesla V100 GPU with the Adam optimizer, where we use an initial learning rate of 0.0001 with a momentum of 0.9. 

\subsection{Baselines}
% \subsubsection{Baselines on Sequence and Plain Graph} 
%Graph Generative Model}
We compare the quality of our hierarchical graph generative model with a sequence generative model in SketchRNN \cite{ha2017neural} and a plain graph generative model PlainGen that derives from the global generation step of \HDMapGen.

\PAR{SketchRNN}. For a sequence generative model, we map all control points of the lane objects inside each HD map into a sequence. Each sequential data point has a pair of 2D coordinates and a state variable to define the continuity of each line. We choose an ascending order of spatial coordinates to define the sequential order. We explore
a conditional and an unconditional variants for this model. For the conditional generation, a target map is provided as both input and target as a variational auto-encoder during training. And it is still provided as an input during sampling. For unconditional generation, a decoder-only model is trained to generate the target maps.

\PAR{PlainGen}.
The plain graph generative model has the same implementation as the global graph generative model in \HDMapGen, and it consumes a plain graph input. Every control point in the map is taken as a node in the plain graph. A corresponding edge is constructed to define whether these two nodes are connected. We use DFS to construct the adjacency matrix and define the order of generation. And we explore two variants of \textit{coordinate-first} and \textit{topology-first} for this model.
%The first baseline we evaluate to test the performance of autoregressive generative model using data representation as sequence is the open source SketchRNN model. 

%The second baseline we have is to apply plain graph generative model. We adopt the same global graph generative model in HDMapGen to perform the generation on the defined plain graph. 






\subsection{Benchmarking Sample Quality}
\subsubsection{Hierarchical Graph Generation}

We evaluate the generation quality and diversity from our hierarchical graph generative model \HDMapGen with three variants of \textit{coordinate-first}, \textit{topology-first} and \textit{independent} with  different  definitions  of  priority  and  dependence on coordinates and topology generation.

\PAR{Global Graph Generation}. We firstly show the generation process of the global graph from \HDMapGen in Figure~\ref{fig: global_graph_generation}. We could see only a small set of global nodes are capable of representing a typical pattern in HD maps to include two parallel crossroads. Meanwhile, we also demonstrate that the diversity of model outputs could be improved with the increasing of the temperature $\tau$. While the diversity and quality trade-off still exist during generation, in our experiments, we find an empirical bound of 0.2 for $\tau$ to guarantee high-quality samples.

\PAR{Local Graph Generation}. %The local graph is generated after each step of a node and corresponding edges are constructed in global graph generation. 
The local graph represent a sequence of control points which reveal the details of each global object. For drivable lanes, the density of control points usually increases at the corner of each lane. And in Figure~\ref{fig: traffic_light}, we show our model is capable of generating such features, and the generated maps always have smooth curves at the corner of each lane.

\PAR{Semantic Attribute Generation}. As shown in  Figure~\ref{fig: traffic_light}, the generated traffic light controlled lanes are mostly located in the cross roads and turn roads. The generated semantic attributes are consistent with the real-world urban scenes. 

\begin{figure}[t]
\begin{center}
%\vspace{-40pt}
\includegraphics[width=1\linewidth]{./figures/paper/global_graph_generation_3.png}
\end{center}
\caption{Top: The global graph autoregressive generative process. Bottom: The diversity of the generated graph is improved when temperature $\tau$ increases. }
%The results are from HDMapGen model trained on the in-house dataset.}
\label{fig: global_graph_generation}
%\vskip -0.3cm
\end{figure}


\begin{figure}[t]
\begin{center}
% %\vspace{-40pt}
\includegraphics[width=1\linewidth]{./figures/paper/traffic_lights.png}
 \end{center}
\caption{Semantic attributes of traffic lights and lanes controlled by traffic light generated from HDMapGen.}
 \label{fig: traffic_light}
 %\vskip -0.3cm
 \end{figure}
 

\begin{figure*}[t]
\begin{center}
\vskip -0.5cm
\includegraphics[width=0.98\linewidth]{./figures/paper/results.png}
\end{center}
\vskip -0.5cm
\caption{Maps with different city styles from hierarchical graph generative models HDMapGen (\textit{coordinate-first}, \textit{topology-first} and \textit{independent}) outperform plain graph generative model PlainGen, and sequence generative model sketchRNN.}
\label{fig: result_baseline}

\end{figure*}



\begin{table*}[t]
\begin{center}
\begin{tabular}{lc|ccc|cc|cc} 
%\hline
\toprule
\multicolumn{2}{c|}{Measurement}&\multicolumn{3}{c|}{Urban Planning} &\multicolumn{2}{c|}{Geometry Fidelity} &\multicolumn{2}{c}{Topology Fidelity}\\
\hline
\multicolumn{2}{c|}{Metrics}&\multicolumn{5}{c|}{Fréchet Distance} &\multicolumn{2}{c}{MMD}\\
\hline
 \multicolumn{2}{c|}{Features} &Conne. &Densi. &Reach. &Len. &Orien. &Deg. &Spec. \\ \cline{1-2}
\multicolumn{2}{c|}{Methods} &$10^{0}$ &$10^{1}$ &$10^{1}$ &$10^{1}$ &$10^{1}$ &$10^{-1}$ &$10^{-1}$\\
\hline
 
 \multirow{2}{*}{SketchRNN} &conditional &0.50 &21.20 &13.43 &2.04 &1.77 &1.03  &4.94 \\ 
  &unconditional &0.44 &41.12 &29.83 &1.64 &1.22 &0.83  &4.74  \\\cline{1-2}
  
 \multirow{2}{*}{PlainGen}  
 &topology-first &0.54 &5.18 &14.57 &1.85 &1.54 &0.17   &0.31  \\ 
 &coordinate-first &0.39 &4.30 &4.81 &1.64 &0.46 &0.12  &\textbf{0.29}  \\\cline{1-2}
 
 \multirow{3}{*}{HDMapGen} &independent &0.31 &4.38 &\textbf{4.22} &\textbf{1.49} &0.52 &0.06 &0.54  \\ 
  &topology-first &0.26 &\textbf{4.06} &4.47 &\textbf{1.49} &\textbf{0.37} &\textbf{0.05} &0.63 \\ 
  &coordinate-first &\textbf{0.17} &4.79 &4.74 &\textbf{1.49} &0.53 &0.07  &0.90 \\ 
\bottomrule
%\hline
\end{tabular}
\end{center}
\caption{Measurements for urban planning, geometry fidelity and topology fidelity for \HDMapGen and baselines PlainGen and SketchRNN. Urban planing (features of connectivity, density and reach) and Geometry (features of the length and orientation of lanes) are quantified with a Fréchet Distance metric.  Topology fidelity (features of node degree and spectrum of graph Laplacian) is quantified with with a MMD metric. For all mertics, lower is better .}
\label{Tab: Quantitative Evaluation}
\end{table*}


\subsubsection{Evaluation Metrics}

We design three measurements to quantify the generation results, including topology fidelity, geometry fidelity, and urban planning statistics.

\textbf{Topology fidelity}. We use maximum mean discrepancy (MMD) [GRAN] to quantify the similarity with real maps on graph statistics using Gaussian kernels with the first Wasserstein distance. The topology statistics we apply here is the degree distributions and spectrum of graph Laplacian.

\textbf{Geometry fidelity}. We use geometry features, the length and orientation of lanes to quantify the similarity with real maps. Then we compute the Fréchet Distance to measure two normal distributions using these features. 
%Such statistics is able to measure the geometry similarity with the target.

\textbf{Urban planning}. We use the common urban planning features, \textit{connectivity} to represent node degree, node \textit{density} within a region, and \textit{reach} as the number of accessible lane within a region to evaluate the transportation plausibility of our generated maps compared with real maps [NTG]. We also use Fréchet Distance to measure two normal distributions of these features. 

%\textbf{Chamfer like distance}: we also use the chamfer like distance to quantify the map-wise similarity of each generative models, and finally provide a measurement of diversity.

\subsubsection{Qualitative and Quantitative Evaluation}

\textbf{Qualitative Evaluation}. In Figure~\ref{fig: result_baseline}, we show the qualitative evaluation for our models and other baselines. The results show that the proposed hierarchical graph generative models HDMapGen (both \textit{coordinate-first} and \textit{topology-first}) generate the highest quality maps, and largely outperform other methods. They capture the typical features of HD maps including the overall layouts, the crossroads and parallel lane patterns, \etc. And they are capable of generating maps with different city styles. For the maps generated from HDMapGen with \textit{independent} model, the crossing of lanes happens frequently as the model fails to take the dependence of coordinates and topology into account. For the plain graph generative model, we find the model completely fail for this task, according to the difficulty to generate a large graph. Since more than ten-fold of edges for each graph are included compared to hierarchical graph. For the sequence generative model SketchRNN, we find the model is available to learn the overall geometric patterns, however, there are a large amount of cut offs or dead ends occurring in the lanes. During the generation of the sequential data, it's possible to stop generating a consecutive point at any step, and then re-start at any arbitrary location. This property is not an issue for a sketch drawing task. Yet for HD map generation, it's important for the model to guarantee the continuity constraint between generated points. 

\textbf{Quantitative Evaluation}. As shown in Table~\ref{Tab: Quantitative Evaluation}, \HDMapGen (both \textit{coordinate-first} and \textit{topology-first}) outperform other baselines on most of the metrics. The results are also consistent with the visualization results. SketchRNN has a poor performance in topology related features, such as degree. According to the issue that cut-offs or dead ends of lanes happen frequently, the generated maps from SketchRNN have a very different distribution of node degree from real maps. PlainGen have a better performance in spectrum of graph Laplacian. As we perform the evaluation for topology features with transforming outputs of all models into the plain graph level, which might preserve the intrinsic topology patterns for outputs from PlainGen.

\subsection{Ablation Studies}
We conduct ablation studies on the impact to use different dependence and generation priority on three variants of \HDMapGen models \textit{coordinate-first}, \textit{topology-first} and \textit{independence}. We show in Table~\ref{tab: ablation_studies}. For \textit{coordinate-first} model, BCE which quantifies the topology prediction performance is the lowest, as after coordinates are generated as a prior, the topology prediction could be better optimized. Meanwhile, for \textit{topology-first} model, the coordinate prediction is better optimized given a generated topology prior. While \textit{independence} model is the worst as it fails to model the dependence of coordinate and topology during generation.   

\begin{table}[h]
\begin{center}
\begin{tabular}{ c c c c}
 \toprule
 Metrics & coordinate-first & topology-first  & independent\\ 
 \hline
 NLL & -5.610  & \textbf{-6.142}  & -4.490\\  
 BCE &\textbf{0.001}  &0.050  & 0.053 \\  
\bottomrule
%\hline
\end{tabular}
\end{center}
\caption{Negative Log likelihood (NLL) and binary cross entropy (BCE) on validation set for HDMapGen with three variants as \textit{coordinate-first}, \textit{topology-first} and \textit{independent}.}
\label{tab: ablation_studies}
\end{table}


\subsection{Performance Evaluation}

We show the time and complexity to generate a map for each model in Table~\ref{tab: performance}. HDMapGen achieves a speed-up of ten-fold compared to SketchRNN. HDMapGen is much more efficient due to (1) the smallest size of adjacency matrix in a representation of hierarchical graph, and (2) utilizing GRAN with the state-of-the-art time-efficiency for global graph generation and a single-shot decoder for local graph generation. 

%GRAN has the  with a complexity of $O(N)$. It outperforms common recurrent models, typically with a complexity of $O(N^2)$.

%will move this to the method part

\begin{table}[h]
%\small
\begin{center}
\begin{tabular}{ c c c c }

 \toprule
 Model & HDMapGen &PlainGen & SketchRNN \\
 \hline
 Time (s) &\textbf{0.20} &0.89 &2.28\\ 
%Complexity &\textbf{$O(N)$} &$O(N^2M)$ &$O(N^2M)$ \\
\bottomrule
\end{tabular}
\end{center}
\caption{Generation time of a map with a FoV of $200m \times
200m$ on HDMapGen, PlainGen and SketchRNN.}
\label{tab: performance}
\end{table}



%\subsection{Comparison of FLOPs and Model Sizes}



==> rebuttal.tex <==
We thank all reviewers for their constructive comments and feedback. Several reviewers mention that the generation task we introduce is novel and valuable (\Ra, \Rb, \Rd), our approach is effective and efficient (\Rb, \Rc, \Rd), and our evaluations are sound and convincing (\Ra, \Rb). Specific concerns are addressed below.

\noindent \textbf{Variety of Generated Maps} [\Ra]
Thanks for mentioning this interesting question.
Our approach and baselines are trained on the same datasets containing many diverse samples. We did not deliberately add any constraint to generate ``grid-like" patterns in our approach. In fact, our model could also generate diverse maps with other acceptable road patterns as revealed in the training sets, which outperforms other methods in evaluation metrics. 

\noindent \textbf{Description and Visualization} [\Rb]
%Thanks for the suggestions. %to improve the presentations.
We will add description of curvature generation for local graph generation, and use a color gradient to represent the generation order. 

\noindent \textbf{Traffic-related Rules} [\Rb]
Thanks for this inspiring question.
Various traffic rules related evaluation methods could be developed, such as transportation \textit{convenience} in Table.~\ref{tab: transportation convenience}, traffic light \textit{density}, driving agents \textit{capacity}.    

\noindent \textbf{Motivation} [\Rc] 
Requiring aerial images to generate does not usually yield novel environments, as these areas have already been mapped. Our work can generate an unlimited amount of diverse maps without requiring high-quality aerial images. Large amounts of HD maps are crucial to train downstream motion forecasting and planning models. %(e.g. https://arxiv.org/abs/1910.05449).

% % Thanks for the questions.
% %We agree that the image-based approach could generate maps for novel environments given aerial images.
% The advantage of our approach is to generate unlimited diverse maps without the need of inputting aerial images.
% %, while only with a small set of annotated HD maps. 
% Meanwhile, an extension on the current approach is to input image embedding to achieve image-based generation, which could be a potential direction in our future work.

\noindent \textbf{Technical Contribution} [\Rc] 
Thanks for the questions, we will include more clarifications on this part. 
\textbf{Sequence representation:} In our model, each local graph represents a directed spline between two control points, so we have a unique order (from the start to the end), and don't have any revisiting issue. \textbf{GRAN:} GRAN is only a component in our model to generate the global topology. We found that other key components we proposed are essential, such as the hierarchical representations, the dependency between topology and geometry during generation, and the efficient local graph decoder. The model most similar to GRAN is the baseline PlainGen, which performs much worse than our approach. \textbf{Plain graph input:} HDmapGen does not require a \textit{plain} graph input. It generates the hierarchical graph by a \textit{global} generator and a \textit{local} graph generator. According to the autoregressive modeling, the \textit{global} graph generator only takes the \textit{global} graph generated from previous steps as inputs. While PlainGen uses the same implementation as the \textit{global} graph generator for \textit{plain} graph generation.
%, it only takes the plain graph generated from previous steps as inputs.

\noindent \textbf{Evaluation} [\Rc] As discussed above, GRAN is not able to generate HD maps, as it only generates the graph topology without geometry information. Meanwhile, PlainGen (a modification of GRAN) is used as a baseline.

\begin{table}[h]
\captionsetup{font=footnotesize}
\setlength{\tabcolsep}{4.8pt}
\begin{center}
\small
\vspace{-2pt}
\begin{tabular}{ c |c c c c c c c c }
\hline
Model &\multicolumn{2}{c|}{SketchRNN} &\multicolumn{2}{c|}{PlainGen} &\multicolumn{3}{c}{HDMapGen}\\ 
%  \hline
Metric &Cond. &\multicolumn{1}{c|}{Uncond.} &ToF. &\multicolumn{1}{c|}{CoF.} & Ind. & ToF. &CoF.\\ 
 \hline
 %&conditional &conditional &topology-first &coordinate-first & independent &topology-first &coordinate-first\\
Conve. &49.4 &49.5 &22.6 &12.0 &11.2 &\textbf{9.9} &11.8 \\
\hline
\end{tabular}
\end{center}
\vspace{-15pt}
\caption{Metric to evaluate the transportation \textit{convenience}. It's calculated as the Fréchet Distance between normal distributions of the Urban Planing Feature (Dijkstra shortest path length for
node pairs) of real and generated maps (scaling by $10^1$).\vspace{-4pt}} 
\vspace{-15pt}
\label{tab: transportation convenience}
\end{table}

\noindent \textbf{Evaluation} [\Rd] 
Thanks for these valuable suggestions.
\textbf{Downstream task:} Since our work is the first to generate fine-grained graphs, developing downstream tasks for evaluation is beyond our current scope, while it's a very interesting direction in the future work. 
\textbf{Metrics:} 1. We will add the transportation \textit{convenience} metric shown in Table.~\ref{tab: transportation convenience} in our revision. It is an adapted version for our task. 2. We find that \textit{Conne.} and \textit{Deg.} are the metrics on which PlainGen has a much worse performance, which is consistent with the qualitative results, where the maps generated from PlainGen lack apparent bifurcation patterns. Meanwhile, we will add NLL on PlainGen, which is three times worse than that of HDMapGen. 3. We will add the corresponding fidelity metrics for our diversity evaluation. The fidelity decreases when the temperature increases. We have an explanation in supp L068. Note that when the temperature is 0, the geometry decoder performs greedy sampling, while the topology decoder still performs non-greedy sampling. In this case, we find the model generates over-simplified maps that are different from the real maps.

\noindent \textbf{Design Choices and Writing Clarity} [\Rd] 
% We appreciate the reviewer for pointing out that more clarifications are needed. 
\textbf{$L_t$ with different dimensions:} We use a padding vector with a fixed maximum length to represent $L_t$, which enables it to be processed with an MLP.  
\textbf{Fine level predictions:} Predicting fine level points can increase the resolution of HD maps. We only generate the intermediate points between control points for the fine-level prediction and use the control points in global graph as vertices to guarantee they begin and end correctly. According to the auto-regressive modeling, we provide the previously generated points as inputs to implicitly avoid self-crossing. As the coarse level quality is more critical in our evaluations, thus the metrics do not change much. \textbf{Starting points:} For both training and evaluation, the start point is randomly selected or sampled for robustness and diversity. 
\textbf{Map patches sampling:} The map patches are sampled randomly, with no bias towards the intersections.
\textbf{Datasets clarification:} We will clarify the datasets for the evaluation numbers in our revision.  
\textbf{Normalization:} The quantities in Table.2 are normalized by graph length (number of generation steps). 

\noindent \textbf{Related Work} [\Rd] 
% Thanks for referring us to these interesting related works in procedure modeling.
We will cite more papers in this area and include more discussion. We agree that it will be interesting to generate maps with different city styles using one model. One extension of our approach is to add a one-hot vector input for city id and train a single model on all datasets, which could be a direction in our future work. 
